The effect of initial texture on multiple necking formation in polycrystalline thin rings subjected to dynamic expansion

In this paper, we have investigated, using finite element calculations, the effect of initial texture on the formation of multiple necking patterns in ductile metallic rings subjected to rapid radial expansion. The mechanical behavior of the material has been modeled with the elasto-viscoplastic single crystal constitutive model developed by \citet{marin2006}. The polycrystalline microstructure of the ring has been generated using random Voronoi seeds. Both $5000$ grain and $15000$ grain aggregates have been investigated, and for each polycrystalline aggregate three different spatial distributions of grains have been considered. The calculations have been performed within a wide range of strain rates varying from $1.66 \cdot 10^4 ~ \text{s}^{-1}$ to $3.33 \cdot 10^5 ~ \text{s}^{-1}$, and the rings have been modeled with four different initial textures: isotropic texture, $\left\langle 001\right\rangle\parallel\Theta$ Goss texture, $\left\langle 001\right\rangle\parallel$ R Goss texture and $\left\langle 111\right\rangle\parallel$ Z fiber texture. The finite element results show that: (i) the spatial distribution of grains affects the location of the necks, (ii) the decrease of the grain size delays the formation of the necking pattern and increases the number of necks, (iii) the initial texture affects the number of necks, the location of the necks, and the necking time, (iv) the development of the necks is accompanied by a local increase of the slip activity. This work provides new insights into the effect of crystallographic microstructure on dynamic plastic localization and guidelines to tailor the initial texture in order to delay dynamic necking formation and, thus, to improve the energy absorption capacity of ductile metallic materials at high strain rates.

==> tmpbib.tex <==
[2.] [1837][1844]
[3.] [923][953]
[4.] [49][70]
[5.] [3555][3580]
[6.] [189][201]
[7.] [183][202]
[10.] [104798][]
[11.] [17][26]
[13.] [1191][1212]
[14.] [1547][1556]
[15.] [393][400]
[16.] [293][306]
[17.] [5615][5632]
[18.] [198][202]
[19.] [401][413]
[20.] [111152][]
[21.] [1001][1008]
[22.] [399][415]
[24.] [1018][1030]
[25.] [135][144]
[27.] [103661][]
[28.] [102999][]
[29.] [1995][2016]
[30.] [300][308]
[31.] [151][160]
[32.] [103418][]
[33.] [29][32]
[34.] [104189][]
[35.] [20170575][]
[36.] [835][844]
[37.] [279][297]
[38.] [012085][]
[39.] [232][236]
[40.] [1729][1745]
[41.] [1357][1376]
[42.] [107][120]
[43.] [799][822]
[44.] [364][368]
[45.] [1199][1202]
[46.] [481][491]
[47.] [134][148]
[48.] [232 ][ 243]
[49.] [109908][]
[50.] [93][113]
[51.] [183][217]
[52.] [3][36]
[53.] [880][891]

